Quantum Monte Carlo study of the two-dimensional fermion Hubbard Model

We report large scale determinant Quantum Monte Carlo calculations of the effective bandwidth, momentum distribution, and magnetic correlations of the square lattice fermion Hubbard Hamiltonian at half-filling. The sharp Fermi surface of the non-interacting limit is significantly broadened by the electronic correlations, but retains signatures of the approach to the edges of the first Brillouin zone as the density increases. Finite size scaling of simulations on large lattices allows us to extract the interaction dependence of the antiferromagnetic order parameter, exhibiting its evolution from weak coupling to the strong coupling Heisenberg limit. Our lattices provide improved resolution of the Green's function in momentum space, allowing a more quantitative comparison with time-of-flight optical lattice experiments.

==> Makefile <==
Target = hub2d-13

#=============================================================================#

LaTeX	= latex
BiBTeX	= bibtex
DVItoPS = dvips -Ppdf -G0 -j0 -t letter
PStoPDF = ps2pdf -dMaxSubsetPct=100 -dCompatibilityLevel=1.3 -dSubsetFonts=true -dEmbedAllFonts=true
FIGS 	= corr.ps corr2.ps corr3.ps excluded_U5.00B20.00_extrap.ps\
	  excluded_U5.00B20.00.ps grad_U2.ps grad_U4.ps greenc_U2.ps\
	  greenc_U4.ps green.ps localmoment.ps order.ps struct.ps teff.ps
FIGS    = fig1.ps fig2.ps fig3.ps fig4.ps fig5.ps fig6.ps fig7.ps\
	  fig8.ps fig9.ps

#=============================================================================#

all:
	@echo "  Specify which option to process"
	@echo "      pdf      - Create PDF (hyperlinked) version"
	@echo "      clean    - Remove temporary files"
	@echo "      cleanall - Remove temporary and output files"
	@echo ""

cleanall:
	rm -f ${Target}.aux ${Target}.bbl ${Target}.blg ${Target}.dvi
	rm -f ${Target}.log ${Target}.lof ${Target}.lot ${Target}.los
	rm -f ${Target}.out ${Target}.toc ${Target}.tpm ${Target}.brf
	rm -f ${Target}.glo ${Target}.gls ${Target}.glg 
	rm -f ${Target}.idx ${Target}.ilg ${Target}.ist
	rm -f ${Target}.ind ${Target}.tpt ${Target}.pdf ${Target}.ps

clean:
	rm -f ${Target}.aux ${Target}.bbl ${Target}.blg ${Target}.dvi
	rm -f ${Target}.log ${Target}.lof ${Target}.lot ${Target}.los
	rm -f ${Target}.out ${Target}.toc ${Target}.tpm ${Target}.brf
	rm -f ${Target}.glo ${Target}.gls ${Target}.glg 
	rm -f ${Target}.idx ${Target}.ilg ${Target}.ist
	rm -f ${Target}.ind ${Target}.tpt 

${Target}.dvi: ${Target}.tex ${FIGS}
	${LaTeX} ${Target}

${Target}.aux: ${Target}.dvi

${Target}.bbl: ${Target}.aux ${Target}.tex
	${BiBTeX} ${Target}.aux

pdf: 	${Target}.bbl ${Target}.tex ${FIGS} hub2d.bib
	${LaTeX} ${Target}
	${LaTeX} ${Target}
	${DVItoPS} ${Target} -o ${Target}.ps
	${PStoPDF} ${Target}.ps


